Signaling in the Age of AI: Evidence from Cover Letters

We study the impact of generative AI on labor market signaling using the introduction of an AI-powered cover letter writing tool on a large online labor platform. Our data track both access to the tool and usage at the application level. Difference-in-differences estimates show that access to the tool increased textual alignment between cover letters and job posts and raised callback rates. Time spent editing AI-generated cover letter drafts is positively correlated with hiring success. After the tool's introduction, the correlation between cover letters' textual alignment and callbacks fell by 51%, consistent with what theory predicts if the AI technology reduces the signal content of cover letters. In response, employers shifted toward alternative signals, including workers' prior work histories.

==> Figures/callback_itt_late.tex <==
\begin{table}[hbtp]
\centering
\caption{Effect of AI on Callbacks}
\label{tab:chatted_regression}
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{c}{Callback} \\
 & (1) ITT & (2) LATE & (3) ITT & (4) LATE \\
\hline
AI & 0.0078*** & 0.0615*** & 0.0038** & 0.0322** \\
   & (0.0016) & (0.0133) & (0.0019) & (0.0159) \\
\hline
Bidder FE & \checkmark & \checkmark & \checkmark & \checkmark \\
Month FE & \checkmark & \checkmark & \checkmark & \checkmark \\
$\text{PostGPT}_t \times \text{Access}_{i}$ &  &  & \checkmark & \checkmark \\
Outcome Mean & 0.0702 & 0.0702 & 0.0702 & 0.0702 \\
Outcome Std. Dev. & 0.2554 & 0.2554 & 0.2554 & 0.2554 \\
\hline
\textit{N} & 2,439,745 & 2,439,745 & 2,439,745 & 2,439,745 \\
\bottomrule
\end{tabular}
\begin{floatnotes}
A callback is defined as being chatted with by the employer after submitting a bid. Columns (1) and (3) report the ITT (the coefficient of PostAI $\times$ Access in the two-way fixed effect specification), while columns (2) and (4) report the LATE, where we instrument for the usage of AI using PostAI $\times$ Access. Columns (1) and (2) omit the PostGPT $\times$ Access term; columns (3) and (4) include it. Wage bids, experience rank percentile, and log bid count are controlled for. Standard errors are clustered at the bidder level. *** p $<$ 0.01, ** p $<$ 0.05, * p $<$ 0.1.
\end{floatnotes}
\end{threeparttable}
\end{table}


==> Figures/complier_characteristics.tex <==
% Generated by freelancer/final/section4/build_adoption_comparison.py
\begin{apptable}
\centering
\captionof{table}{Comparison of Pre-Period Observables by AI Tool Use}
\label{tab:complier_characteristics}
\begin{threeparttable}
\renewcommand{\arraystretch}{0.82}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrrr}
\toprule
\toprule
 & Never used & Ever used & Difference & SMD \\
\midrule
\multicolumn{5}{l}{\textit{Panel A. Bidder-Level}} \\
\hspace{0.75em}Weeks Active & 5.792 & 8.052 & 2.260 & 0.512 \\
\hspace{0.75em}Bids per Active Week & 9.296 & 25.369 & 16.073 & 0.422 \\
\hspace{0.75em}Cover Letter Tailoring & 0.116 & 0.125 & 0.008 & 0.086 \\
\hspace{0.75em}Normalized Wage Bid & 3.165 & 3.228 & 0.063 & 0.035 \\
\hspace{0.75em}Experience Score & 0.755 & 0.782 & 0.027 & 0.184 \\
\hspace{0.75em}Callback Rates & 0.095 & 0.080 & -0.0145 & -0.102 \\
\hspace{0.75em}Awarded Rates & 0.014 & 0.013 & -0.0004 & -0.007 \\
\hspace{0.75em}$N$ & 1{,}467 & 2{,}386 & - & - \\
\midrule
\multicolumn{5}{l}{\textit{Panel B. Bid-Level}} \\
 & Non-AI bids & AI bids & Difference & SMD \\
\hspace{0.75em}Cover Letter Tailoring & 0.116 & 0.122 & 0.006 & 0.070 \\
\hspace{0.75em}Normalized Wage Bid & 3.550 & 3.509 & -0.040 & -0.033 \\
\hspace{0.75em}Experience Score & 0.867 & 0.855 & -0.012 & -0.091 \\
\hspace{0.75em}Callback Rates & 0.075 & 0.070 & -0.0051 & -0.091 \\
\hspace{0.75em}Awarded Rates & 0.007 & 0.007 & 0.0002 & 0.011 \\
\hspace{0.75em}$N$ & 1{,}209{,}401 & 190{,}692 & - & - \\
\bottomrule
\bottomrule
\end{tabular}
\begin{floatnotes}
This table is restricted to workers with access at rollout in the DiD estimation sample. Tool use is measured from April 19 to September 15, 2023. Panel A compares workers who used the tool at least once with those who never used it during that period, weighting each bidder equally. Its characteristics are measured from January 19 to April 18, 2023. Panel B compares post-rollout AI-assisted and unassisted bids, attaching each bidder's pre-period averages to every bid; all characteristics therefore remain measured before rollout, and each post-rollout bid receives equal weight. The same bidder may contribute to both bid groups. Weeks active counts pre-period weeks with at least one sample bid; bids per active week divides pre-period bids by weeks active. Experience score summarizes past work and reviews; wages are normalized by the minimum job budget. Difference is Ever used minus Never used in Panel A and AI bids minus Non-AI bids in Panel B. SMD divides the difference by the square root of the average of the two group sample variances. $N$ counts bidders in Panel A and post-rollout bids in Panel B.
\end{floatnotes}
\end{threeparttable}
\end{apptable}


==> Figures/cover_letter_tailoring_heterogeneity.tex <==
\begin{table}[hbtp]
\centering
\caption{Heterogeneous Effect of AI on Cover Letter Tailoring}
\label{tab:tfidf_heterogeneity}
\begin{threeparttable}
\begin{tabular}{lcc}
\toprule
 & \multicolumn{2}{c}{Cover Letter Tailoring} \\
\cmidrule(lr){2-3}
 & (1) & (2) \\
\hline
$\text{Post}_t \times \text{Access}_i$ & 0.0255*** & 0.0209*** \\
 & (0.0032) & (0.0032) \\
$\text{Post}_t \times \text{Access}_i \times \text{Pre-AI Ability}_i$ & -0.0112** & -0.0112** \\
 & (0.0045) & (0.0045) \\
\hline
Bidder FE & \checkmark & \checkmark \\
Month FE & \checkmark & \checkmark \\
$\text{PostGPT}_t \times \text{Access}_{i}$ &  & \checkmark \\
Outcome Mean & 0.1508 & 0.1508 \\
Outcome Std. Dev. & 0.1639 & 0.1639 \\
\hline
\textit{N} & 2,439,745 & 2,439,745 \\
\bottomrule
\end{tabular}
\begin{floatnotes}
The table reports regression results with cover letter tailoring as the outcome. Heterogeneous effects are based on the worker's standardized average cover letter tailoring in the period before the AI tool was introduced. Column (2) additionally controls for a PostGPT $\times$ Treat term. Wage bids, experience rank percentile, and log job-level bid count are controlled for. Standard errors are reported in parentheses and clustered at the bidder level. *** p $<$ 0.01, ** p $<$ 0.05, * p $<$ 0.1.
\end{floatnotes}
\end{threeparttable}
\end{table}


==> Figures/cover_letter_tailoring_itt_late.tex <==
\begin{table}[hbtp]
\centering
\caption{Effect of AI on Cover Letter Tailoring}
\label{tab:tfidf_regression}
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{c}{Cover Letter Tailoring} \\
 & (1) ITT & (2) LATE & (3) ITT & (4) LATE \\
\hline
AI & 0.0256*** & 0.2017*** & 0.0209*** & 0.1765*** \\
   & (0.0032) & (0.0190) & (0.0032) & (0.0200) \\
\hline
Bidder FE & \checkmark & \checkmark & \checkmark & \checkmark \\
Month FE & \checkmark & \checkmark & \checkmark & \checkmark \\
$\text{PostGPT}_t \times \text{Access}_{i}$ &  &  & \checkmark & \checkmark \\
Outcome Mean & 0.1508 & 0.1508 & 0.1508 & 0.1508 \\
Outcome Std. Dev. & 0.1639 & 0.1639 & 0.1639 & 0.1639 \\
\hline
\textit{N} & 2,439,745 & 2,439,745 & 2,439,745 & 2,439,745 \\
\bottomrule
\end{tabular}
\begin{floatnotes}
Cover letter tailoring is measured as textual similarity--the cosine similarity between TF-IDF vectors of a cover letter and a job description. Columns (1) and (3) report the ITT (the coefficient of PostAI $\times$ Access in the two-way fixed effect specification), while columns (2) and (4) report the LATE, where we instrument for the usage of AI using PostAI $\times$ Access. Columns (1) and (2) omit the PostGPT $\times$ Access term; columns (3) and (4) include it. Wage bids, experience rank percentile, and log bid count are controlled for. Standard errors are clustered at the bidder level. *** p $<$ 0.01, ** p $<$ 0.05, * p $<$ 0.1.
\end{floatnotes}
\end{threeparttable}
\end{table}


==> Figures/eventstudy_combined.tex <==
\begin{table}[hbtp]
\centering

\caption{Predictive Power of Bid Characteristics Before and After AI}
\label{tab:eventstudy_combined}
\begin{threeparttable}
\begin{tabular}{lcc}
\toprule
& Callback & Offer \\
\midrule
$\text{Cover Letter Tailoring}_{ijt}$
& 0.036603*** & 0.003382*** \\
& (0.002383) & (0.000658) \\
$\text{Post}_t \times \text{Cover Letter Tailoring}_{ijt}$
& -0.018942*** & -0.003401*** \\
& (0.002605) & (0.000677) \\

\midrule

$\text{Experience Score}_{ijt}$
& 0.058666*** & -0.004349*** \\
& (0.007388) & (0.001666) \\
$\text{Post}_t \times \text{Experience Score}_{ijt}$
& 0.013035*** & -0.000116 \\
& (0.004076) & (0.000758) \\

\midrule

$\text{Normalized Wage Bid}_{ijt}$
& -0.001754*** & -0.000212*** \\
& (0.000101) & (0.000027) \\
$\text{Post}_t \times \text{Normalized Wage Bid}_{ijt}$
& -0.000167* & 0.000011 \\
& (0.000098) & (0.000021) \\

\midrule
Bidder FE & \checkmark & \checkmark  \\
Month FE & \checkmark & \checkmark  \\
\midrule
\textit{N} & 5{,}651{,}635 & 5{,}651{,}635 \\
\bottomrule
\end{tabular}
\begin{floatnotes}
The table reports bid-level regressions that include all three bid characteristics and their interactions with the post-AI indicator. Cover-letter tailoring is the cosine similarity between the TF-IDF vectors of the cover letter and job post. Experience score is a platform-calculated score based on the volume and strength of a bidder's past reviews. Normalized wage is the bid amount divided by the project's minimum budget. Bidder and month fixed effects are included. Log job-level bid count is controlled for. Standard errors are reported in parentheses and clustered at the bidder level.  *** p $<$ 0.01, ** p $<$ 0.05, * p $<$ 0.1.
\end{floatnotes}
\end{threeparttable}

\end{table}


==> Figures/preperiod_balance.tex <==
\begin{table}
\centering
\caption{Comparison of Pre-period Observables between Treatment and Control Workers}
\label{tab:preperiod_balance}
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
\toprule
Variable & Control mean & Treated mean & Diff.\ $(T-C)$ & SMD \\
\midrule
Weeks Active & 2.32 & 7.19 & 4.87 & 1.36 \\
Bids per Active Week & 2.08 & 19.2 & 17.2 & 0.587 \\
Cover Letter Tailoring & 0.112 & 0.122 & 0.00969 & 0.0891 \\
Normalized Wage Bid & 3.04 & 3.20 & 0.168 & 0.0898 \\
Experience Score & 0.594 & 0.772 & 0.178 & 1.51 \\
Callback Rate & 0.0721 & 0.0860 & 0.0139 & 0.0848 \\
Award Rate & 0.00752 & 0.0132 & 0.00573 & 0.0968 \\
\midrule
Bidders & 14{,}395 & 3{,}853 & \multicolumn{2}{l}{Total = 18{,}248} \\
\bottomrule
\bottomrule
\end{tabular}
\begin{floatnotes}
This table reports pre-treatment bidder-level averages for workers included in the DiD estimation sample, separately for control and treated workers. Experience score is a platform-calculated score summarizing workers' work histories. Normalized wage bid is bid normalized by the job's minimum budget. Diff.\ (T-C) denotes the treated mean minus the control mean. SMD denotes the standardized mean difference.
\end{floatnotes}
\end{threeparttable}
\end{table}

